On the Dynamics of Point Vortices with Positive Intensities collapsing with the boundary

In this paper, we study the point-vortex dynamics with positive intensities. We show that in the half-plane and in a disk, collapses of point vortices with the boundary in finite time are impossible, hence the solution of the dynamics is global in time. We also give some necessary conditions for the existence of collapses with the boundary in general smooth bounded domains, in particular, that the trajectory of at least one point vortex has no limit. Some minor results are obtained with unsigned intensities.

==> commandes.tex <==

%%% Complexes

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\cu}{\mathbf{i}}


%%% Proba

\newcommand{\Cov}{\text{Cov}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\Esp}{\mathbb{E}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\ps}{\text{ p.s. }}
\newcommand{\pp}{\text{ p.p. }}
\newcommand{\Tloi}[2]{\stackrel{\mathrm{loi}}{\tend{#1}{#2}}}
\newcommand{\Tps}[2]{\stackrel{\mathrm{p.s.}}{\tend{#1}{#2}}}
\newcommand{\TProb}[2]{\stackrel{\mathrm{\mathbb{P}}}{\tend{#1}{#2}}}

%%% Analyse

\newcommand{\tend}[2]{\underset{#1\to #2}{\longrightarrow} }
\newcommand{\limite}[2]{\lim\limits_{#1 \rightarrow #2}}

\newcommand{\norm}[2]{{\left\|#1\right\|}_{#2}}
\newcommand{\ntriple}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\scal}[2]{\left\langle #1 \, , \, #2 \right\rangle }

\newcommand{\loc}{\mathrm{loc}}

\newcommand{\Ent}[1]{{\lfloor #1 \rfloor}}

%\newcommand{\dist}{\mathrm{dist \, }}
\DeclareMathOperator\dist{dist} 

\newcommand{\der}[2]{\frac{\dd #1}{\dd #2}}
\newcommand{\parder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pparder}[3]{\frac{\partial^{#3} #1}{\partial #2}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\Diff}{\mathrm{D}}

\newcommand{\sign}{\mathrm{sign}}
\newcommand{\supp}{\mathrm{supp}\hspace{1mm}}
\newcommand{\complem}{^\mathsf{c}}
\newcommand{\diam}{\hspace{0.2mm}\mathrm{diam}\hspace{1mm}}
\newcommand{\curl}{\hspace{0.2mm}\mathrm{curl}\hspace{1mm}}
\renewcommand{\div}{\hspace{0.2mm}\mathrm{div}\hspace{1mm}}
\newcommand{\arcl}{\hspace{0.2mm}\mathrm{arclength}\hspace{1mm}}



\newcommand{\eps}{\varepsilon}
\newcommand{\cst}{\mathrm{cst}}


%%% Ensembles

\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Rd}{{\R^d}}
\newcommand{\Rn}{{\R^n}}

%%% Typo

\newcommand{\ds}{\displaystyle}
\newcommand{\vs}{\vspace{1mm}}
\renewcommand{\sp}{\hspace{0.2cm}}




%%% Méca flu

\newcommand{\tgm}{\tilde{\gamma}}
\renewcommand{\tilde}{\widetilde}

%%% Théorèmes
\theoremstyle{plain}
	\newtheorem{theorem}{Theorem}[section]
	\newtheorem{proposition}[theorem]{Proposition}    
	\newtheorem{lemma}[theorem]{Lemma}          
	\newtheorem{corollary}[theorem]{Corollary}
	\newtheorem{conjecture}[theorem]{Conjecture}
	
\theoremstyle{definition}
	\newtheorem{definition}[theorem]{Definition}


%%% Lettres

%%%%%% Raccourcis lettres calligraphiées
\def\cA{{\mathcal A}} \def\cB{{\mathcal B}} \def\cC{{\mathcal C}} 
\def\cD{{\mathcal D}} \def\cE{{\mathcal E}} \def\cF{{\mathcal F}} 
\def\cG{{\mathcal G}} \def\cH{{\mathcal H}} \def\cI{{\mathcal I}} 
\def\cJ{{\mathcal J}} \def\cK{{\mathcal K}} \def\cL{{\mathcal L}} 
\def\cM{{\mathcal M}} \def\cN{{\mathcal N}} \def\cO{{\mathcal O}} 
\def\cP{{\mathcal P}} \def\cQ{{\mathcal Q}} \def\cR{{\mathcal R}} 
\def\cS{{\mathcal S}} \def\cT{{\mathcal T}} \def\cU{{\mathcal U}} 
\def\cV{{\mathcal V}} \def\cW{{\mathcal W}} \def\cX{{\mathcal X}} 
\def\cY{{\mathcal Y}} \def\cZ{{\mathcal Z}} 

%%%%%% Raccourcis lettres gothiques
\def\mA{{\mathfrak A}} \def\mB{{\mathfrak B}} \def\mC{{\mathfrak C}} 
\def\mD{{\mathfrak D}} \def\mE{{\mathfrak E}} \def\m{{\mathfrak F}} 
\def\mG{{\mathfrak G}} \def\mH{{\mathfrak H}} \def\mI{{\mathfrak I}} 
\def\mJ{{\mathfrak J}} \def\mK{{\mathfrak K}} \def\mL{{\mathfrak L}} 
\def\mM{{\mathfrak M}} \def\mN{{\mathfrak N}} \def\mO{{\mathfrak O}} 
\def\mP{{\mathfrak P}} \def\mQ{{\mathfrak Q}} \def\mR{{\mathfrak R}} 
\def\mS{{\mathfrak S}} \def\mT{{\mathfrak T}} \def\mU{{\mathfrak U}} 
\def\mV{{\mathfrak V}} \def\mW{{\mathfrak W}} \def\mX{{\mathfrak X}} 
\def\mY{{\mathfrak Y}} \def\mZ{{\mathfrak Z}} 

%%% Commandes Ludo mathcal

\def\AA{{\mathbb A}} \def\BB{{\mathbb B}} \def\CC{{\mathbb C}} 
\def\DD{{\mathbb D}} \def\EE{{\mathbb E}} \def\FF{{\mathbb F}} 
\def\GG{{\mathbb G}} \def\HH{{\mathbb H}} \def\II{{\mathbb I}} 
\def\JJ{{\mathbb J}} \def\KK{{\mathbb K}} \def\LL{{\mathbb L}} 
\def\MM{{\mathbb M}} \def\NN{{\mathbb N}} \def\OO{{\mathbb O}} 
\def\PP{{\mathbb P}} \def\QQ{{\mathbb Q}} \def\RR{{\mathbb R}} 
\def\SS{{\mathbb S}} \def\TT{{\mathbb T}} \def\UU{{\mathbb U}} 
\def\VV{{\mathbb V}} \def\WW{{\mathbb W}} \def\XX{{\mathbb X}} 
\def\YY{{\mathbb Y}} \def\ZZ{{\mathbb Z}} 


%%% Couleur pour remarques
\newcommand{\martin}[1]{\texttt{\color{violet} #1}}
\newcommand{\ludovic}[1]{\texttt{\color{blue} #1}}
\newcommand{\dragos}[1]{\texttt{\color{red} #1}}
